VoxelNet: End-to-End Learning for Point Cloud Based 3D Object Detection

Accurate detection of objects in 3D point clouds is a central problem in many applications, such as autonomous navigation, housekeeping robots, and augmented/virtual reality. To interface a highly sparse LiDAR point cloud with a region proposal network (RPN), most existing efforts have focused on hand-crafted feature representations, for example, a bird's eye view projection. In this work, we remove the need of manual feature engineering for 3D point clouds and propose VoxelNet, a generic 3D detection network that unifies feature extraction and bounding box prediction into a single stage, end-to-end trainable deep network. Specifically, VoxelNet divides a point cloud into equally spaced 3D voxels and transforms a group of points within each voxel into a unified feature representation through the newly introduced voxel feature encoding (VFE) layer. In this way, the point cloud is encoded as a descriptive volumetric representation, which is then connected to a RPN to generate detections. Experiments on the KITTI car detection benchmark show that VoxelNet outperforms the state-of-the-art LiDAR based 3D detection methods by a large margin. Furthermore, our network learns an effective discriminative representation of objects with various geometries, leading to encouraging results in 3D detection of pedestrians and cyclists, based on only LiDAR.

==> Section_Discussion.tex <==
\section{Discussion}

==> Section_RelatedWork.tex <==


%However, these manually-designed feature representations introduce an information bottleneck that constrains these approaches from effectively exploiting 3D shape information and required invariances for the detection task. 

%Multi-modality fusion is another promising direction for 3D object detection~\cite{REF:Enzweiler2011,REF:Gonzalez2017,REF:cvpr17chen}. However, in this work we aim to push the limit of point-cloud-based 3D detection and therefore do not elaborate on this topic.

